View-consistent 4D Light Field Depth Estimation

We propose a method to compute depth maps for every sub-aperture image in a light field in a view consistent way. Previous light field depth estimation methods typically estimate a depth map only for the central sub-aperture view, and struggle with view consistent estimation. Our method precisely defines depth edges via EPIs, then we diffuse these edges spatially within the central view. These depth estimates are then propagated to all other views in an occlusion-aware way. Finally, disoccluded regions are completed by diffusion in EPI space. Our method runs efficiently with respect to both other classical and deep learning-based approaches, and achieves competitive quantitative metrics and qualitative performance on both synthetic and real-world light fields

==> bibliography.tex <==
@inproceedings{anonymous2020,
    author={Anonymous},
    title={Fast and Accurate 4D Light Field Depth Estimation},
    booktitle={submission; included as supplemental material},
    year={2020},
}

@inproceedings{jiang2019,
  author={Xiaoran Jiang and Jinglei Shi and Christine Guillemot},
  title={A learning based depth estimation framework for 4D densely and sparsely sampled light fields},
  booktitle={Proceedings of the 44th International Conference on Acoustics, Speech, and Signal Processing (ICASSP)},
  year={2019}
}

@article{chen2018,
  title={Accurate light field depth estimation with superpixel regularization over partially occluded regions},
  author={Chen, Jie and Hou, Junhui and Ni, Yun and Chau, Lap-Pui},
  journal={IEEE Transactions on Image Processing},
  volume={27},
  number={10},
  pages={4889--4900},
  year={2018},
  publisher={IEEE}
}


@inproceedings{alperovich2018,
  author    = {A. Alperovich and O. Johannsen and B. Goldluecke},
  title     = {Intrinsic Light Field Decomposition and Disparity Estimation with a Deep Encoder-Decoder Network},
  booktitle = {26th European Signal Processing Conference (EUSIPCO)},
  year      = {2018}
}

@article{barnes09,
   author   = "Connelly Barnes and Eli Shechtman and Adam Finkelstein and Dan B Goldman",
   title    = "{PatchMatch}: A Randomized Correspondence Algorithm for Structural
      Image Editing",
   journal  = "ACM Transactions on Graphics (Proc. SIGGRAPH)",
   year     = "2009",
   month    = aug,
   volume   = "28",
   number   = "3"
}

@INPROCEEDINGS{bhat2009,
    AUTHOR  = "Pravin Bhat and Larry Zitnick and Michael Cohen and Brian Curless",
    TITLE   = "GradientShop: A Gradient-Domain Optimization Framework for Image and Video Filtering",
    booktitle = "ACM Transactions on Graphics (TOG)",
    YEAR    = 2009
}

@ARTICLE{chuchvara2020,
author  = {A. {Chuchvara} and A. {Barsi} and A. {Gotchev}},
journal = {IEEE Transactions on Image Processing (TIP)},
title   = {Fast and Accurate Depth Estimation From Sparse Light Fields},
year    = {2020},
volume  = {29},
number  = {},
pages   = {2492-2506}
}

%% Bibtex entry URL: bibtexbrowser_html.php?key=AJG18%3Aeusipco&bib=self.bib

@inproceedings{ha2016,
  title     = {High-quality depth from uncalibrated small motion clip},
  author    = {Ha, Hyowon and Im, Sunghoon and Park, Jaesik and Jeon, Hae-Gon and So Kweon, In},
  booktitle = {IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  pages     = {5413--5421},
  year      = {2016}
}

@inproceedings{heber2016,
  title.    = {Convolutional networks for shape from light field},
  author.   = {Heber, Stefan and Pock, Thomas},
  booktitle = {IEEE Conference on Computer Vision and Pattern Recognition},
  pages     = {3746--3754},
  year      = {2016}
}

@inproceedings{honauer2016,
  title     = {A dataset and evaluation methodology for depth estimation on 4D light fields},
  author    = {Honauer, Katrin and Johannsen, Ole and Kondermann, Daniel and Goldluecke, Bastian},
  booktitle = {Asian Conference on Computer Vision},
  pages     = {19--34},
  year      = {2016},
  organization = {Springer}
}

@inproceedings{holynski2018,
    author    = {Aleksander Holynski and Johannes Kopf},
    title     = {Fast Depth Densification for Occlusion-aware Augmented Reality},
    booktitle = {ACM Transactions on Graphics (Proc.~SIGGRAPH Asia)},
    publisher = {ACM},
    volume    = {37},
    number    = {6},
    year      = 2018}
}

@inproceedings{huang18,
  title     = {Deep{MVS}: Learning Multi-view Stereopsis},
  author    = {Huang, Po-Han and Matzen, Kevin and Kopf, Johannes and Ahuja, Narendra and Huang, Jia-Bin},
  booktitle = {IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  pages     = {2821--2830},
  year      = {2018}
}

@inproceedings{ilg2017,
  title     = {Flownet 2.0: Evolution of optical flow estimation with deep networks},
  author    = {Ilg, Eddy and Mayer, Nikolaus and Saikia, Tonmoy and Keuper, Margret and Dosovitskiy, Alexey and Brox, Thomas},
  booktitle = {IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  pages     = {2462--2470},
  year      = {2017}
}


@inproceedings{jeon2015,
  title       = {Accurate depth map estimation from a lenslet light field camera},
  author      = {Jeon, Hae-Gon and Park, Jaesik and Choe, Gyeongmin and Park, Jinsun and Bok, Yunsu and Tai, Yu-Wing and So Kweon, In},
  booktitle   = {IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  pages       = {1547--1555},
  year        = {2015}
}

 
@inproceedings{jiang2018,
  title     = {Depth estimation with occlusion handling from a sparse set of light field views},
  author    = {Jiang, Xiaoran and Le Pendu, Mika{\"e}l and Guillemot, Christine},
  booktitle = {25th IEEE International Conference on Image Processing (ICIP)},
  pages     = {634--638},
  year      = {2018},
  organization = {IEEE}
}

@inproceedings{khan2019,
  title     = {View-consistent {4D} Light Field Superpixel Segmentation},
  author    = {Khan, Numair and Zhang, Qian and Kasser, Lucas and Stone, Henry and Kim, Min H. and Tompkin, James},
  booktitle = {International Conference on Computer Vision (ICCV)},
  year      = {2019},
  organization = {IEEE}
}

@techreport{khan2020,
  title     = {Fast and Accurate {4D} Light Field Depth Estimation},
  author    = {Khan, Numair and Kim, Min H. and Tompkin, James},
  year      = {2020},
  institution = {Brown University},
  number      = {CS-20-01},
}

@inproceedings{ma2013,
  title={Constant time weighted median filtering for stereo matching and beyond},
  author={Ma, Ziyang and He, Kaiming and Wei, Yichen and Sun, Jian and Wu, Enhua},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision},
  pages={49--56},
  year={2013}
}


@inproceedings{rerabek2016,
  title     = {New Light Field Image Dataset},
  author    = {Rerabek, Martin and Ebrahimi, Touradj},
  booktitle = {8th International Conference on Quality of Multimedia Experience (QoMEX)},
  number    = {CONF},
  year      = {2016}
}

        
@article{shi2019,
  title     = {A framework for learning depth from a flexible subset of dense and sparse light field views},
  author    = {Shi, Jinglei and Jiang, Xiaoran and Guillemot, Christine},
  journal   = {IEEE Transactions on Image Processing (TIP)},
  volume    = {28},
  number    = {12},
  pages     = {5867--5880},
  year      = {2019},
  publisher = {IEEE}
}

@inproceedings{Shih2020,
  author = {Shih, Meng-Li and Su, Shih-Yang and Kopf, Johannes and Huang, Jia-Bin},
  title = {3D Photography using Context-aware Layered Depth Inpainting},
  booktitle = {IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  year = {2020}
}

@inproceedings{shin18,
  title     = {Epinet: A fully-convolutional neural network using epipolar geometry for depth from light field images},
  author    = {Shin, Changha and Jeon, Hae-Gon and Yoon, Youngjin and So Kweon, In and Joo Kim, Seon},
  booktitle = {IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  pages     = {4748--4757},
  year      = {2018}
}

@incollection{szeliski2006,
  title     = {Locally adapted hierarchical basis preconditioning},
  author    = {Szeliski, Richard},
  booktitle = {ACM SIGGRAPH 2006 Papers},
  pages     = {1135--1143},
  year      = {2006}
}


@inproceedings{tao2013,
  title     = {Depth from combining defocus and correspondence using light-field cameras},
  author    = {Tao, Michael W and Hadap, Sunil and Malik, Jitendra and Ramamoorthi, Ravi},
  booktitle = {IEEE International Conference on Computer Vision (ICCV)},
  pages     = {673--680},
  year      = {2013}
}

@misc{stanford2008,
title = {{The New Stanford Light Field Archive}}, 
url   = {http://lightfield.stanford.edu/}, 
publisher = {Stanford Graphics Laboratory}, 
year={2008}
} 

@inproceedings{tosic2014,
  title     = {Light field scale-depth space transform for dense depth estimation},
  author    = {Tosic, Ivana and Berkner, Kathrin},
  booktitle = {IEEE Conference on Computer Vision and Pattern Recognition Workshops (CVPRW)},
  pages     = {435--442},
  year      = {2014}
}


@inproceedings{wang15,
  title={Occlusion-aware depth estimation using light-field cameras},
  author={Wang, Ting-Chun and Efros, Alexei A and Ramamoorthi, Ravi},
  booktitle={IEEE International Conference on Computer Vision (ICCV)},
  pages={3487--3495},
  year={2015}
}

@article{wang16,
  title={Depth Estimation with Occlusion Modeling using Light-field Cameras},
  author={Wang, Ting-Chun and Efros, Alexei A and Ramamoorthi, Ravi},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence (TPAMI)},
  volume={38},
  number={11},
  pages={2170--2181},
  year={2016},
  publisher={IEEE}
}

@inproceedings{wanner2012,
  title     = {Globally consistent depth labeling of 4D light fields},
  author    = {Wanner, Sven and Goldluecke, Bastian},
  booktitle = {IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  pages     = {41--48},
  year      = {2012},
  organization = {IEEE}
}

@article{wanner2013,
  title     = {Variational light field analysis for disparity estimation and super-resolution},
  author    = {Wanner, Sven and Goldluecke, Bastian},
  journal   = {IEEE transactions on pattern analysis and machine intelligence},
  volume    = {36},
  number    = {3},
  pages     = {606--619},
  year      = {2013},
  publisher = {IEEE}
}

@incollection{wilburn2005,
  title={High performance imaging using large camera arrays},
  author={Wilburn, Bennett and Joshi, Neel and Vaish, Vaibhav and Talvala, Eino-Ville and Antunez, Emilio and Barth, Adam and Adams, Andrew and Horowitz, Mark and Levoy, Marc},
  booktitle={ACM SIGGRAPH 2005 Papers},
  pages={765--776},
  year={2005}
}

@inproceedings{yucer2016,
  title.       = {Depth from gradients in dense light fields for object reconstruction},
  author       = {Yucer, Kaan and Kim, Changil and Sorkine-Hornung, Alexander and Sorkine-Hornung, Olga},
  booktitle    = {4th International Conference on 3D Vision (3DV)},
  pages        = {249--257},
  year         = {2016},
  organization = {IEEE}
}

@article{zhang2016,
  title     = {Robust depth estimation for light field via spinning parallelogram operator},
  author    = {Zhang, Shuo and Sheng, Hao and Li, Chao and Zhang, Jun and Xiong, Zhang},
  journal   = {Computer Vision and Image Understanding},
  volume    = {145},
  pages     = {148-159},
  year      = {2016}
}

